AnaMeta: A Table Understanding Dataset of Field Metadata Knowledge Shared by Multi-dimensional Data Analysis Tasks

Tabular data analysis is performed every day across various domains. It requires an accurate understanding of field semantics to correctly operate on table fields and find common patterns in daily analysis. In this paper, we introduce the AnaMeta dataset, a collection of 467k tables with derived supervision labels for four types of commonly used field metadata: measure/dimension dichotomy, common field roles, semantic field type, and default aggregation function. We evaluate a wide range of models for inferring metadata as the benchmark. We also propose a multi-encoder framework, called KDF, which improves the metadata understanding capability of tabular models by incorporating distribution and knowledge information. Furthermore, we propose four interfaces for incorporating field metadata into downstream analysis tasks.

==> 7-discussions.tex <==


% \subsection{Real-world Deployment}
\label{sec:deployment}
By automatic recognition of table metadata, automatic analysis can be conducted. With large corpus and smart supervision mentioned in \refsec{sec:corpora}, We have worked with a leading IT company and deployed a simplified version of the tree-based metadata model as a fundamental spreadsheet table understanding APIs. The model is integrated with intelligent features, such as one-click data analysis (insights mining\cite{ding2019quickinsights}),  natural language QA, pivot table, and charts recommendation in its product.
% \TODO{See Justin's paper}


% \subsection{Extending Analysis Metadata}
% There are far more types of analysis metadata to be discovered and inferred. On the one hand, inspired by data profiling metadata, the dependency between multi-fields in one table plays an important role. There are several common dependencies or relationships among columns. How to identify them is future work.
% On the other hand, in \reftab{tab:msr-taxonomy} only a limited taxonomy is provided. A more comprehensive one is future work.


% \subsection{Tabular Model Improvements}
% %As discussed in \refsec{sec:exp}, several existing approaches on tabular modeling all have improvement space in the future. There is still an efficiency gap for real-world deployment of large pre-trained tabular models in products. 
% Understanding numbers in tables and designing proper pre-train objectives is still a challenge for us to explore. 
% %Meanwhile, feature engineering seems inevitable in tabular models at current stage. 
% Further explorations on semantic and distributional features are still needed.

% Utilizing existing knowledge graph information to interpret and analyze table is important and promising. We make the first attempt in this work, and it's still a future work.

